Weighted Minwise Hashing Beats Linear Sketching for Inner Product Estimation

We present a new approach for computing compact sketches that can be used to approximate the inner product between pairs of high-dimensional vectors. Based on the Weighted MinHash algorithm, our approach admits strong accuracy guarantees that improve on the guarantees of popular linear sketching approaches for inner product estimation, such as CountSketch and Johnson-Lindenstrauss projection. Specifically, while our method admits guarantees that exactly match linear sketching for dense vectors, it yields significantly lower error for sparse vectors with limited overlap between non-zero entries. Such vectors arise in many applications involving sparse data. They are also important in increasingly popular dataset search applications, where inner product sketches are used to estimate data covariance, conditional means, and other quantities involving columns in unjoined tables. We complement our theoretical results by showing that our approach empirically outperforms existing linear sketches and unweighted hashing-based sketches for sparse vectors.

==> table-2-example.tex <==
\begin{figure}[t]
% \def\arraystretch{1.0}
% \scriptsize
\centering
\footnotesize
% \small
\parbox{1.0\linewidth}{
\setlength{\tabcolsep}{0.35em}
\begin{tabular}{c|cccccccccccccccc}
\toprule
% & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 \\
index & \bf 1 & \bf 2 & \bf 3 & \bf 4 & \bf 5 & \bf 6 & \bf 7 & \bf 8 & \bf 9 & \bf 10 & \bf 11 & \bf 12 & \bf 13 & \bf 14 & \bf 15 & \bf 16 \\
\midrule
$\bv{x}^{V_A}$ & 6.0 &0  & 2.0 & \bf 6.0 & \bf 1.0 & 4.0 & 2.0 & \bf 2.0 & 8.0 & 0 & \bf 3.0 & 0 & 0 & 0 & 0 & 0 \\
$\bv{x}^{\ind{K_A}}$ & 1 & 0 & 1 & \bf 1 & \bf 1 & 1 & 1 & \bf 1 & 1 & 0 & \bf 1 & 0 & 0 & 0 & 0 & 0 \\
\midrule
$\bv{x}^{V_B}$ & 0   & 1.0 &0  & \bf 5.0 & \bf 1.0 &0  &0  & \bf 2.0 & 0 & 4.0 & \bf 2.5 & 6.0 & 0 & 0 & 6.0 & 3.7 \\
$\bv{x}^{\ind{K_B}}$ &	0 & 1 & 0 & \bf 1 & \bf 1 & 0 & 0 & \bf 1 & 0 & 1 & \bf 1 & 1 & 0 & 0 & 1 & 1 \\
\bottomrule
\end{tabular}
}
\vspace{-1em}

\caption{
Vector representation of tables $\mathcal{T}_A$ with $\mathcal{T}_B$ from Figure~\ref{fig:example-tables}. The vector $\bv{x}^{\ind{K_A}}$ (resp. $\bv{x}^{\ind{K_B}}$) is the vector representation for the join key $K_A$ (resp. $K_B$) and $\bv{x}^{V_A}$ (resp. $\bv{x}^{V_B}$) is the vector representation for the column $V_A$ (resp. $V_B$). Bold numbers are entries included in the join result $\mathcal{T}_{A \bowtie B}$.
}
\vspace{-2em}
\label{fig:ex-vectors}
\end{figure}


